Density-aware NeRF Ensembles: Quantifying Predictive Uncertainty in Neural Radiance Fields

We show that ensembling effectively quantifies model uncertainty in Neural Radiance Fields (NeRFs) if a density-aware epistemic uncertainty term is considered. The naive ensembles investigated in prior work simply average rendered RGB images to quantify the model uncertainty caused by conflicting explanations of the observed scene. In contrast, we additionally consider the termination probabilities along individual rays to identify epistemic model uncertainty due to a lack of knowledge about the parts of a scene unobserved during training. We achieve new state-of-the-art performance across established uncertainty quantification benchmarks for NeRFs, outperforming methods that require complex changes to the NeRF architecture and training regime. We furthermore demonstrate that NeRF uncertainty can be utilised for next-best view selection and model refinement.

==> nerf.tex <==

\section{A Review of the NeRF Rendering Equation}
We start with revisiting the foundational NeRF rendering equation from Mildenhall et al.~\cite{mildenhall2021nerf}.
Given a ray $\vr(t) = \vo + t\vd$ with origin point $\vo$ and direction $\vd$, the expected colour $C(\vr)$ of camera ray $\vr(t)$ with near and far bounds $t_n$ and $t_f$ is:
\begin{equation}
    C(r) = \int_{t_n}^{t_f} T(t) \cdot \rho(r_{(t)}) \cdot \vc(\vr_{(t)}, \vd) \;dt.
\end{equation}
This integral has three components: $T(t)$ is the accumulated transmittance along the ray from $t_n$ to $t$, i.e. the probability that the ray travels from $t_n$ to $t$ without hitting another particle. It describes how much light is attenuated as it travels back to the camera. It is calculated as: 
\begin{equation}
    T(t) = \exp \left( -\int_{t_n}^{t}\rho(\vr_{(s)})\;ds  \right).
\end{equation}
The density $\rho(r_{(t)})$ denotes to the differential probability that a ray interacts with the volumetric medium of the scene at a particular point. $\rho(r_{(t)})$ is not a probability, but a density that can take on values greater than 1. Lastly, $\vc(\vr_{(t)}, \vd)$ denotes the predicted colour at the point $\vr_{(t)}$ seen from direction $\vd$.

In practice these integrals are approximated via the quadrature rule, using sums and stratified sampling from $N$ evenly spaced bins to make the rendering process tractable:
\begin{equation}
    C(\vr) = \sum_{i=1}^N T_i \cdot \big(1-\exp(-\rho_i\delta_i)\big) \cdot \vc_i, 
    \label{eq:render_sum}
\end{equation}
Now $1-\exp(-\rho_i\delta_i)$ is the probability of the $i$-th bin being occupied. As before, $T_i$ is the transmittance, this time calculated using discrete summation instead of continuous integration:
\begin{equation}
    T_i = \exp\left(-\sum_{j=1}^{i-1}\rho_j\delta_j\right),
\end{equation}
and $\delta_i = t_{i+1} - t_i$ is the distance between adjacent samples. The complete rendering equation for a single ray is therefore given as:
\begin{equation}
    C(\vr) = \sum_{i=1}^N \exp\left(-\sum_{j=1}^{i-1}\rho_j\delta_j\right) \cdot \big(1-\exp(-\rho_i\delta_i)\big) \cdot \vc_i.
\end{equation}


Following the rule that $\exp(a+b) = \exp(a) \cdot \exp(b)$, we can rewrite the transmittance as a product: 
\begin{equation}
    \label{eq:transmittance_prod}
    T_i = \prod_{j=1}^{i-1} \exp(-\rho_j\delta_j).
\end{equation}
Combining equations (\ref{eq:transmittance_prod}) and (\ref{eq:render_sum}), we can express the full rendering equation for a single ray as
\begin{equation}
    C(\vr) = \sum_{i=1}^N \prod_{j=1}^{i-1} \exp(-\rho_j\delta_j)  \cdot \big(1-\exp(-\rho_i\delta_i)\big)  \cdot \vc_i, 
\end{equation}
By writing the occupancy probability $1-\exp(-\rho_i\delta_i)$ as $o_i$, this becomes the convenient expression
\begin{equation}
    C(\vr) = \sum_{i=1}^N 
    \overbrace{
        \underbrace{\prod_{j=1}^{i-1} (1-o_j)}_\text{transmittance}
        \cdot 
        \underbrace{o_i}_\text{occupancy}  
    }^\text{termination probability}
    \cdot 
    \overbrace{\vc_i}^\text{colour}
    \label{eq:render}
\end{equation}

